Domain Adaptation and Entanglement: an Optimal Transport Perspective

Current machine learning systems are brittle in the face of distribution shifts (DS), where the target distribution that the system is tested on differs from the source distribution used to train the system. This problem of robustness to DS has been studied extensively in the field of domain adaptation. For deep neural networks, a popular framework for unsupervised domain adaptation (UDA) is domain matching, in which algorithms try to align the marginal distributions in the feature or output space. The current theoretical understanding of these methods, however, is limited and existing theoretical results are not precise enough to characterize their performance in practice. In this paper, we derive new bounds based on optimal transport that analyze the UDA problem. Our new bounds include a term which we dub as \emph{entanglement}, consisting of an expectation of Wasserstein distance between conditionals with respect to changing data distributions. Analysis of the entanglement term provides a novel perspective on the unoptimizable aspects of UDA. In various experiments with multiple models across several DS scenarios, we show that this term can be used to explain the varying performance of UDA algorithms.

==> figures/table_acc_summary.tex <==
\begin{table*}[htbp]
    \label{table1}
    \centering
    \small
    \caption{%
        Performance of different algorithms including the LJE oracle objective minimization tested over various distribution shift scenarios. Each cell reports ``source accuracy / target accuracy'' and approaches with positive transfer (\ie, better than ERM) are notated by an underline \underline{x} and the best overall method is notated by a box \fbox{y}.
        (Top table) presents the best model \emph{conv1} and (Bottom table) presents a selection of other model results.
        }    
    \vspace{0.1cm}
    \begin{tabular}{lccccc}
    \toprule
     Scenario + Best Model & LJE Oracle & ERM & WRR & JDOT & DANN \\
     \midrule
     MNIST $\to$ USPS / conv1 & 97.6 / 94.7 & 98.0 / 83.8 & 96.9 / \underline{86.0} & 98.2 / \underline{87.1} & 96.2 / \fbox{89.3} \\
     %
     USPS $\to$ MNIST / conv1 & 95.2 / 98.0 & 94.8 / 71.4 & 94.8 / \underline{78.8} & 95.6 / \fbox{89.3} &  93.3 / \underline{77.9} \\
     %
     MNIST $\to$ MNIST-M / conv1 & 99.2 / 96.8 & 98.9 / 47.5 & 98.8 / \underline{51.2} & 99.1 / \underline{69.3} & 98.8 / \fbox{79.1} \\
     %
     SVHN $\to$ MNIST / conv1 & 92.3 / 99.1 & 91.2 / 64.9 & 90.4 / \fbox{65.3} & 90.4 / 48.0 & 86.6 / 10.3 \\
     %
     Portraits $1905\text{-}1974 \to 1974\text{-}2013$ / conv1 & 96.9 / 95.5 & 96.8 / 86.3 & 94.8 / 83.8 & 96.5 / 85.2 & 95.8 / \fbox{87.3} \\
     %
     CIFAR10 $\to$ CIFAR10c / conv1 & 72.7 / 83.8 & 75.5 / 37.7 & 71.2 / 10.0 & 10.0 / 10.0 & 73.7 / \fbox{60.9} \\
     \bottomrule
    \end{tabular}

    \vspace{0.5cm}
    
    \begin{tabular}{lccccc}
    \toprule
     Scenario + Other Models & LJE Oracle & ERM & WRR & JDOT & DANN \\
     \midrule
     MNIST $\to$ USPS / MLP & 92.4 / 91.4 & 92.6 / 16.0 & 90.8 / \fbox{59.3} & 92.4 / \underline{37.8} & 91.4 / \underline{28.8} \\
     %
     USPS $\to$ MNIST / MLP & 92.7 / 94.7 & 91.8 / 29.0 & 90.3 / \fbox{52.1} & 92.3 / \underline{50.5} & 91.6 / \underline{43.1} \\
     %
     MNIST $\to$ MNIST-M / LeNet & 98.7 / 94.5 & 98.9 / 48.4 & 93.6 / \underline{56.3} & 99.0 / \fbox{58.5} & 89.6 / 19.9 \\
     %
     SVHN $\to$ MNIST / conv2 & 90.9 / 98.9 & 90.1 / 64.4 & 19.6 / 11.3 & 90.6 / \fbox{68.7} & 80.6 / 18.7 \\
     %
     Portraits $1905\text{-}1974 \to 1974\text{-}2013$ / MLP & 94.8 / 90.5 & 94.5 / 83.5 & 90.9 / 77.9 & 94.6 / \fbox{84.1} & 94.6 / 83.0 \\
     %
     CIFAR10 $\to$ CIFAR10c / small$\_$cnn & 67.4 / 88.0 & 70.3 / 39.6 & 58.2 / 10.0 & 10.0 / 10.1 & 68.3 / \fbox{52.7} \\
     %     
     \bottomrule
    \end{tabular}
   % 
   % 
   % 
   % 
   % 
    %Domain adaptation experiment results according to the best model \emph{conv1} (top table), a CNN with six convolutional layers followed by two fully connected layers, and other models (bottom table) that are sampled from a much bigger set of experiments in the Appendix. Results suggest that entanglement depends on the (model, dataset, optimizer) triplet, and seemingly the best model or the best method, can easily degrade to chance-level accuracy whenever the other two factors change for the worse.}
\end{table*}


==> figures/table_oracle_summary.tex <==
\begin{table*}[t!]
  \centering
  \small
    \caption{Comparison of the accuracy of minimizing LJE and $\CCA$ with quantities associated with the WRR objective. Cells formatted as X / Y correspond to the metric evaluated on the source / target data. $W_1(\hat{p}_y, \hat{q}_y)$ corresponds to the empirical Wasserstein distance between the marginal label distributions. The values under the ``Oracle Accuracy" header correspond to the accuracy values. The values under ``WRR" correspond to empirical estimates of the accuracy, risk, WRR objective and label-entanglement, respectively.}
    \vspace{0.1cm}
  \scalebox{0.95}{  
  \begin{tabular}{lccccccc}
    \toprule
    \multirow{2}*{Scenario + Model} & \multirow{2}*{$W_{1}(\hat{p}_{\rm y}, \hat{q}_{\rm y})$} & \multicolumn{2}{c}{Oracle Accuracy} & \multicolumn{4}{c}{WRR} \\
    %{Scenario + Model} & {$W_{1}(\hat{p}_y, \hat{q}_y)$} & \multicolumn{3}{c}{Oracle Accuracy} & \multicolumn{3}{c}{WRR} \\
    %\cmidrule(lr){1-1}
    %\cmidrule(lr){2-2}
    \cmidrule(lr){3-4}
    \cmidrule(lr){5-8}
    & & $\LJE$ & $\CCA$ & Acc. & $\hat{\risk}_p$ / $\hat{\risk}_q$ & $\hat{\wrr}$ & $\hat{\labelentangle}$ \\
    \midrule
    MNIST $\to$ USPS / conv1 & 0.13 & 97.6 / 94.7 & 95.3 / 93.0 & 98.5 / 91.7 & 0.06 / 0.15 & 0.23 & 0.08 \\
    %
    MNIST $\to$ USPS / MLP & 0.13 & 92.4 / 91.4 & 93.1 / 87.9 & 95.6 / 74.3 & 0.14 / 0.42 & 0.37 & 0.19 \\
    %
    MNIST $\to$ MNIST-M / conv1  & 0.00 & 99.2 / 96.8 & 98.6 / 95.3 & 98.8 / 70.7 & 0.02 / 0.42 & 0.19 & 0.30 \\
    %
    SVHN $\to$ MNIST / conv2 & 0.20 & 90.9 / 98.9 & 86.8 / 93.9 & 89.1 / 64.8 & 0.19 / 0.50 & 0.38 & 0.34 \\
    %
    Portraits $1905\text{-}1974 \to 1974\text{-}2013$ MLP & 0.05 & 94.8 / 90.5 & 91.6 / 87.3 & 94.0 / 79.6 & 0.09 / 0.29 & 0.11 & 0.33 \\
    %
    CIFAR10 $\to$ CIFAR10c / conv1 & 0.00 & 75.2 / 87.2 & 63.7 / 9.9 & 73.9 / 9.7 & 0.48 / 1.13 & 0.77 & 0.58 \\
    %    
    \bottomrule
  \end{tabular}
  }
  \label{table2}
\end{table*}


==> rebuttal.tex <==
\clearpage

\section{Rebuttal}
\subsection{General reply}

We thank the reviewers (noted as R1-5 below, corresponding to reviewers pBhN, 8ycN, GAmG, 4Jsd and dggm, respectively) for taking the time to read our submission, and for their continued effort throughout the rebuttal process. We would like to summarize here the reviews and our response.

Among the strengths of the paper, all reviewers mentioned that we provide new theoretical results. Our theoretical analysis and generalization bounds were appreciated in general by the reviewers (R2, R3, R5 in particular). The overall organization was found to be clear by most reviewers (R1, R2, R5) and some reviewers highlighted that the paper is well written and very clear (R2 and R5). Some reviewers mentioned we offered a more complete understanding of UDA compared to existing works (R5) and that we properly justified the superiority of our entanglement-based framework over the commonly adopted frameworks in the literature (R1). 

The experiments were seen by at least one reviewer as supporting the theoretical contributions of the paper (R5) but some reviewers were confused (R1) about the take-home messages from the results shown in Tables 1 and 2. R2 requested some clarification about the experiments and R3 and R4 requested experiments to be extended (with more baselines and larger scale datasets). Equally importantly, R1 raised some concerns about the relation to the existing related work, in particular in relation to the conditional discrepancy terms introduced in the literature. Finally, some reviewers questioned the feasibility of our assumptions 1, 2 and 3 (metric and bounded loss, and surjectivity of the model, respectively) or would have liked a more detailed discussion (R3, R5).

Based on the above points, we will improve the paper quality by:
\begin{enumerate}
    \item Extending the related work section significantly. We will add a separate subsection discussing the conditional discrepancy terms introduced in the literature and highlight our contributions appropriately in the light of this existing work. Due to space constraints, a lot of discussion was relegated to the Appendix (section E). We will connect these two sections better, streamlining the discussion.
    \item We will extend the experiments section including a new baseline (reverse-KL) and a larger scale dataset (tiny-Imagenet). Similarly to the above point, due to space constraints, a lot of detailed discussion including accuracy plots corresponding to Tables 1 and 2 were relegated to the Appendix (section F). We will connect these two sections better. We will stress the take-home messages from Tables 1 and 2 more clearly in the main text.
    \item We discuss our assumptions 1-3 in detail in the Appendix (section D). The main text (section 3.1) however, does not link to this section. We will modify the main text accordingly and streamline the discussion.
    Additionally, we note that whilst going through the reviews, we have discovered Assumption 3 can be replaced by a significantly simpler and almost trivial to satisfy assumption. An assumption that the hypothesis space consists of measurable function is all that is required to have the same results in the paper. A sketch of the modifications required are provided in our response to Reviewer GAmG.
    \item We will add minor modifications throughout the text to address other minor concerns that were raised, e.g., we will improve the caption and the figure in Figure 1. We went over the text again and found a few typos, we will fix them.
\end{enumerate}

Would the reviewers be able to raise their scores? Thank you very much in advance.

\subsection{Individual replies}

\paragraph{Reply to reviewer pBhN.}

We thank the reviewer for the insightful comments and the references mentioned. 
Below we try to answer the concerns raised.

% \fix{Many notations are introduced to define the learning framework under entanglement and optimal transport, where a simplification for notations could be helpful to improve the readability.}

% We went over the next carefully but we were not able to identify any notation which could be simplified.

\fix{There is a slight abuse of conditional distributions in entanglement terms. For example, in Def. 3.3, when the distributions are related to the predicted variable $\hat{y} = f(x)$, the subscript of distribution is $y \mid f$ or $f \mid y$ (which seems should be $y \mid \hat{y}$ or $\hat{y} \mid y$).}

We thank the reviewer for their recommendation on the change in notation. We agree that $y \mid f$ is a cumbersome choice. However, 
we introduced this notation in order to emphasize the dependence of the \emph{label-entanglement} on the hypothesis $f$ and believe that this justifies the more complicated notational choice. We will clarify this further in the updated manuscript.

\fix{The experiment part is somewhat hard to follow for me. Specifically, as far as I understand this paper, the key is to evaluate the superiority of the entanglement term-based rules, i.e., Wasserstein distance regularized source risk minimization (WRR) and close conditionals assumption (CCA). However, from the experiment results in Tab. 1 and Tab. 2, these rules seem to be inferior to the existing LJE rule.}

% Table 1 -> LJE is the ceiling, and the ceiling is lower with CCA
% CCA provides a lower ceiling, a tighter bound, for e.g. CIFAR10
% With DANN it is harder to disentangle the min-max optimization 
% Point them to the figures in the Appendix where the ceiling is clearer
We apologize for the confusion that the experiments section caused. Table 1 is meant to show that there is no clear winner among different domain matching algorithms (such as WRR) that do not use target labels: that is due to the entanglement of conditionals (more precisely, the \emph{label-entanglement}) that can happen during the matching process. The \emph{LJE oracle} approach simply applies ERM using both source and target labels, i.e., tries to minimize $\emprisk_p(f) + \emprisk_q(f)$ using stochastic gradient descent. It is there to show the limits of the adaptation process, e.g., it is not reasonable to expect any unsupervised domain adaptation algorithm to exceed $83.8 \%$ accuracy on the CIFAR10c dataset using the conv1 model.

Having argued that the WRR method (that does not have access to the target labels, and hence cannot evaluate the entanglement terms) is not \emph{worse} than other (non-oracle) methods, we take a closer look at WRR in Table 2 in order to instantiate our bounds that use the label entanglement. Using the Euclidean distance as the loss function (in order to avoid scaling the entanglement term) we show that our bounds provide reasonably tight bounds on the target accuracy of the model optimized by WRR after ten epochs. The oracles LJE and CCA, as in Table 1, are here to show the limits of what we should expect from the WRR adaptation procedure. CCA as the oracle minimizing $\emprisk_p(f) + \max_y W_{1, \ell}(f \# p(x|y), f \# q(x|y))$ provides a tighter ceiling than LJE for the target accuracy of domain matching algorithms, e.g., we should not expect the WRR optimized model to exceed $9.9 \%$ accuracy in the CIFAR10c dataset.

The above points become clearer perhaps when taken together with the plots shown in Appendix (Figures 2-4 in section F), where, e.g., the limiting nature of the oracles are more apparent. We will improve our presentation of the experimental results such that the above points are made clearer in the main text.

\fix{An important issue is that some important references (which share the same spirit with the defined entanglement term) are missing, which could reduce the significance of the contribution. Specifically, the differences between the derived results and existing results are expected to be clarified from the following aspects:

1. The entanglement terms essentially imply conditional discrepancy on $f(x) \mid y$ or $y \mid f(x)$, where the marginal terms in bounds become $y$ or $f(x)$, respectively. Such decomposition forms are known as generalized label shift or generalized covariate shift, which are well studied in existing literature, e.g., generalized label shift theory (Thm. 3.1, r1) for and information-theoretic decomposition (Eq. (3) and Prop. 5, r2) for $y \mid f(x)$.

2. The conditional discrepancy bound under optimal transport theory has been studied by Kirchmeyer et al. (Thm. 1, r3), where the 1-Wasserstein-based bounds with similar form are also provided, i.e., marginal discrepancy on
and conditional discrepancy on $f(x) \mid y$ are reflected by Alignment (A) and Label (L), respectively.

Therefore, the core idea of entanglement seems to have been presented in existing works, where the merits are less significant.}

We thank the reviewer for the references mentioned and apologize for the oversight in coverage of past related work. We did mention an important reference \cite{zhao2019learning} in the main text introducing\footnote{Actually the \emph{average conditional discrepancy} term was introduced first in Theorem 1 of \cite{benDavid2010}, however it was not used in the central theorem of that paper that utilized the $H \Delta H$-divergence, and the contribution of \cite{zhao2019learning} lay precisely in connecting the two theorems together.} the average conditional discrepancy, replacing the joint error $\lambda^{\star}$ of \cite{benDavid2010}. However it is true that we were too economical in our literature review, partially due to lack of space in the main text. 

We went over the references mentioned carefully:

1. In Combes et al., the Error Decomposition Theorem 3.1 forms a counterpart to the Theorem 4.1 in \cite{zhao2019learning}, in that Theorem 4.1 of \cite{zhao2019learning} corresponds to the one direction of Lemma 2 in our paper (Wasserstein distance between the model outputs + label entanglement), while Theorem 3.1 of Combes et al. corresponds to the other direction (Wasserstein distance between the labels + prediction entanglement). The authors use the second direction to come up with a weighted risk minimization algorithm similar to other IW-based methods proposed in the literature to handle label shift [du Plessis et al.], while we used the second direction only for theoretical analysis in section 4. %Optimal Transport literature also proposes algorithms which do modify optimal transport to tackle label shift [\new{TODO: citation needed}] in a similar manner. - is this needed?

% Zhao et al., On Learning Invariant Representation for Domain Adaptation \\
% Combes et al., Domain Adaptation with Conditional Distribution Matching and Generalized Label Shift \\
% du Plessis et al., Semi-Supervised Learning of Class Balance under Class-Prior Change by Distribution Matching

Generalized Label Shift (GLS) assumption is a sufficient condition that enforces zero (prediction) entanglement, and in general is not feasible to achieve without target labels (as can be seen by the dependency of the upper bound in Theorem 3.4 of Combes et al. on the target risk). This is also highlighted in the third reference that was mentioned. The entanglement terms, as we wrote in the introduction, capture the hardness of UDA (from an information-theoretic perspective) in a concise but general way: during any domain matching procedure that does not have access to target labels, the optimized model $f$ may entangle the conditionals (in the output space) hence we cannot expect any assumptions such as GLS to be a useful guide during this optimization. 

% \new{Add one more sentence in support of the generality of our proposed framework: the associations computed during the domain matching procedure (optimal transport in this case) are included directly in the bound, as opposed to previous terms in e.g., \cite{zhao2019learning} where the connection is less clear.} 

% chain rule
% Wang and Mao also uses similar chain rule
2. Federici et al. uses the KL-divergence chain rule (an equality) to introduce their concept shift / conditional discrepancy terms. These are based on the KL-divergence and its symmetric counterpart the JS-divergence, both of which require the shared support assumption, unlike the optimal-transport based bounds that we derive, which are more general. We did compare our bound in a remark in Appendix C to the KL-divergence equality (which also appears in \cite{nguyen2022kl} that was already cited) and we will highlight the connection more strongly in the paper.
% which requires shared-support as mentioned and hence is not directly useful for probability distributions that do not share support (such as those found in standard deep learning datasets like MNIST or CIFAR).
% \fix{Alex: Careful here. Although f-divergences require shared support, there seems to be many practical examples of them outperforming IPM based methods, eg, KL-Guided paper. It may be better to consider this a "scope" issue of the paper. Although, ofc, connection exist due to Pinker's inequality etc. Although, because of this IPMs should be tighter, but sometimes perform worse?
% Also, in KL guided paper, they utilize a variational representation. This "deals" with non-zero support issues at the cost of working with probabilistic NNs.}

% Our result seems to be more general and would imply (2) of the 3rd reference
% simpler (less assumptions since we don't include algorithmic framework), more general (we cover both directions) and together with Theorem of section 3 we can infer (2)
3. The third reference, as mentioned by the reviewer, is more relevant, as they include the Wasserstein distance as the discrepancy term of choice. The mentioned bounds are in the context of an algorithm that does not perform domain matching per se (instead it belongs to the family of \emph{asymmetric} approaches (see, e.g., Zhuang et al) but learns a transformation between the two domains. More specifically, the authors learn a transformation $\phi$ (parameterized as a separate neural network) between the source and target embeddings $z$, together with the label proportions $p_N^{Y}$. The label term (L) in the bound does not correspond to the effect of entanglement but rather to the effect of the misestimation of label proportions $p_T^{Y}$. 

The authors by making assumptions 1-4, get rid of any conditional discrepancy terms in the bound that would correspond to our entanglement. Similarly to GLS, these assumptions, especially assumption 3, may be too prohibitive in a lot of cases. The distributions that satisfy Assumption 3 correspond to a type of mild distribution shift. This is to be contrasted to our assumption of Gradual Shift, which together with Probabilistic Margin Assumptions allows one to control/bound the effects of entanglement in Theorem 4.7.

We apologize for the wordy response. To summarize, our bounds handle the more general case in which entanglement plays an important role during the optimization and cannot be neglected. In the revised manuscript we will extend the Related Works section with a subsection on the conditional discrepancy terms introduced in the literature and relate our contributions to those papers, in the light of the discussion above. 

\paragraph{Reply to reviewer 8ycN.}

We thank the reviewer for the comments and the positive evaluation. Below we try to address your concerns.

\fix{It is not clear why the experiments are run with 10 epochs.}

As we argue in the Ablations section (Appendix G): "In this article, we highlighted the (model, dataset, optimizer) dependency of entanglement. This triple dependency has severe consequences for UDA: changes in target accuracy can be attributed to hyperparameters, model selection, algorithmic choices or dataset selection (e.g. label shift removal)."
Indeed, setting the number of epochs as $10$, similar to other hyperparameters and model configurations, has an effect on the UDA performance, which we tried to highlight in the Ablations section by pointing out the consequences of training for more epochs in the USPS $\to$ MNIST scenario. 

Overall any take-home messages from the two tables shown in the results section should be independent of this hyperparameter. As we argued also in our reply to Reviewer pBhN, the results in Table 1 are meant to show that there is no clear winner among different domain matching algorithms (such as WRR) that do not use target labels. This point holds for arbitrary settings of the number of epochs parameter, as evidenced by the results section and the further ablations. Likewise, the results in Table 2 and the points that we highlight in the main text are independent of the number of epochs.
\new{To drive the point home, we might want to run other algorithms as well for more epochs in the Ablations section.}

\fix{The number of experiments, e.g., for table 1 and table 2, as well as the standard deviations of those metrics, is unknown.}

Due to lack of space in the tables we decided to put the details of these experiments to Appendix F. As we write in Appendix F under the Plots subsection: "In Figures 2 to 4 we pick three scenario/model cases to present target accuracy errorbar plots for each method shown in Table 1. We present mean +/- standard deviations over three different seeds, ..." Similarly, "In Figures 5 and 6 we show three scenario/model cases for the method WRR using the Euclidean distance as the loss function. These scenario/model cases correspond to the results shown in Table 2."

We thank the reviewer for bringing up the above points. We will make sure that the sections F and G (Experimental Details and Ablations sections, respectively) are better connected with the results section of the main text.

\fix{All related works are cited but the discussion is less clear.}

We will try to make the Related Works discussion more clear by extending the section in the main text and better streamlining with the extended discussion in Appendix E. More specifically, we will add more recent references and highlight the novelty of the introduced entanglement terms and the CCA assumption, as a stronger assumption than LJE required to be satisfied for the success of UDA algorithms. Moreover, as we wrote in our reply to reviewer pBhN, we will include (in a separate subsection) a discussion on the conditional discrepancy terms introduced and discussed in the literature. 

\paragraph{Reply to reviewer GAmG.}

We thank the reviewer for the insightful review and hope to address the concerns raised.

\fix{One major concern is the weak implications of entanglement-based theoretical results. It is unclear in what situations the entanglement term can be a better tool for analyzing the optimization landscape of UDA algorithms compared to Low Joint Error. Subsection 4.1 discusses imbalanced learning, but this scenario is not involved in the experiments.}

% Entanglement term reflects what happens in practice more clearly - descriptive
% This is what theory can do without further assumption and is 'descriptive'
The entanglement terms (and in general the conditional discrepancy terms introduced e.g. in \cite{zhao2019learning}), as we argued in the main text, highlight the the need to use \emph{stable} as opposed to \emph{spurious} features, and connects UDA to frameworks such as Invariant Risk Minimization \cite{arjovsky2019invariant} that try to learn stable features (i.e., ones that generalize to different target distributions.) In the case of Optimal Transport, the label entanglement term that we introduce, unlike the best joint error of \cite{benDavid2010} and \cite{courty2017}, explicitly depends on the optimal transport map aligning the marginal distributions, which suggests algorithmic approaches as a result.

Based on the Gradual Shift assumption, we tried to indicate one direction that an algorithmic framework could follow: by ensuring Gradual Shift is maintained in the embedding / output space (where the UDA optimization is being done) one could limit the effect of entanglement (by keeping it suitably bounded). Alternatively, a regularized OT framework could try to dampen entanglement (unknown without target labels but perhaps estimated through unsupervised means): and several works in the literature do mention the importance of regularizing OT suitably from a practical perspective. \new{[Citation needed.]}

These are algorithmic directions that are beyond the scope of this paper, but are exciting directions to follow up in future work. We tried to indicate some of these directions in the Conclusion section, and we will expand the text based on this discussion.

\fix{There are two major types of unsupervised domain adaptation algorithms: minimizing the marginal distribution shifts (e.g., DANN) and minimizing joint distribution shifts (e.g., JDOT). More recent baselines can be included to analyze how the entanglement can be applied to analyze the optimization landscape of UDA algorithms, e.g., explaining whether the second type of UDA algorithm has better performance.}

Although JDOT in the original paper \cite{courty2017} is motivated with the goal of minimizing joint distributions shifts, we would like to clarify that the proposed algorithm in the end tries to align only the marginal distributions (in the output and optionally, in the intermediate layers).

Generalizing, we think there is only one type of domain matching algorithm for UDA and that is the marginal type. In our opinion, what differentiates JDOT from adversarial approaches such as DANN is not so much the type of distributions that they hope to match, but rather the algorithmic means they employ towards the UDA goal (of having high target accuracy). 

We added two new baselines: MMD (see e.g. [1]) and a more recent baseline which we call as \emph{reverse-KL} (based on the paper [2]). 

\new{Include the results as a table here}.


The reverse-KL algorithm similarly to JDOT matches marginal distributions (using KL-divergence minimization, as opposed to optimal transport) but similar to JDOT, the authors in the paper discuss how such a marginal alignment can contribute to the overall goal of maintaining high target accuracy (JDOT by making Probabilistic Lipschitzness and LJE assumption, and reverse-KL by making several assumptions highlighted in the text, including the shared-support assumption, which we think is not a feasible assumption to make for most datasets.)

We will make the above points clearer when we introduce and discuss the algorithms in the Results section and in the corresponding Appendix F.

[1] Li, Ya, et al. "Domain generalization via conditional invariant representations." Proceedings of the AAAI conference on artificial intelligence. Vol. 32. No. 1. 2018.

\fix{The explanation of the illustration example in Figure 1 can be improved. The color of the data points is unclear. How does this figure show that entanglement measures the average loss of associating pairs with different labels?}

% Include a legend (give bullet list of changes)
% Maybe add another figure showing a good case where entanglement is low
We agree that Figure 1 can be improved. In the figure, we tried to show an example pair of images corresponding to an association computed by optimal transport in the output space of a convolutional neural network during the WRR-based adaptation. Optimal Transport associates a female image to a male image, possibly because the network is using spurious features (relying on statistically dominant features such as hair length and shape) to represent these images. 

We will improve this figure and point out the colors of the data points.

\fix{Assumption 1 shows the requirements of the loss function, e.g., symmetric and triangle inequality. It is more convincing to provide some commonly used loss examples to explain how the derived theoretical results can be applied in real applications.}

In Section 3.1 of the main text we pointed out that: "Assumption~\ref{assum:metric} is commonly made in the DA literature, in particular, the symmetry and triangle inequality properties of the loss function are often utilized to factor out terms involving the best model $f^{\star}$ (minimizing the source and target risk jointly)~\citep{benDavid2010}. When optimal transport is additionally utilized~\citep{courty2017} to bound the target risk the identity of indiscernibles also needs to hold. % --- if $\ell$ satisfies Lipschitz continuity, this identity must hold.

It should be noted although symmetry can be accounted for via symmetrizing the loss function -- \eg, $\tilde{\ell}(y, y') = \frac{1}{2} (\ell(y, y') + \ell(y', y))$ -- not all symmetric loss functions will satisfy the triangle inequality. Despite this, Assumption~\ref{assum:metric} can be replaced with an \emph{approximate triangle inequality}~\citep{crammer2008learning} with slight alteration to our results. A previous discussion of this weakened assumption in DA was made in \citet[Appendix B.10]{wang2022information}."
Section D in our Appendix continues this discussion and details how our results extend to more commonly used loss functions that do not obey triangle inequality. We realize that we did not refer to this section of the Appendix in the main text, we will update the discussion accordingly such that the two discussions are connected.

% Boundedness of the loss function you can't get around it - it needs to be at least satisfied for the
% distributions of interest.

\fix{Assumption 3 shows the surjective function. How can this assumption be guaranteed for model, e.g., neural networks used in the experiments?}

\new{We thank the reviewer for their question about our surjectivity assumption. The assumption is indeed a difficult assumption to hold in practice. However, we have recently found a way to circumvent this difficult assumption. Instead, all our result follow with only the following assumption: We only require our models to be surjective to a measurable subset $\mathcal{B} \subseteq \mathcal{Y}$. As one would expect our models in practice to be measurable, this assumption will automatically hold (pre-image of measurable function is measurable).

To be more concrete on how this relaxation can be made, we highlight what the original surjective assumption was used for.
In our paper, surjectivity was to ensure that the pushforward of $f$ was a surjective operation on transport measures (following \citet[Theorem 1.101]{leskela2010stochastic}, this was incorrectly referenced in the submitted version of the text and will be corrected in the next version). Instead, we can consider restriction on the codomain; and with additional technical arguments, one can recover the usual Wasserstein distances.

A proof sketch:
We modify the proof of Lemma 3.1 after defining $\bar{f}$ (for simplicity of the rebuttal, we will abuse notation to have $f = \bar{f}$ whenever appropriate).
$f$ now is only surjective on $\mathcal{B}$. Thus we are surjective on transport plans on restricted inputs $\mathcal{B}$. Precisely, as per the proof of Lemma 3.1, let us denote $\Gamma$ denote the set of transport plans and $\Gamma_{\mid \mathcal{B}} \subset \Gamma$ denote a subset of the transport plans with support only on $\mathcal{B}$. Now restricted surjectivity on $f$ tells us that for any $\bar{\gamma} \in \Gamma_{\mid \mathcal{B}}(f\#p, f\# q)$, there exists a $\gamma' \in \Gamma_{\mid \mathcal{B}}(p, q) \subset \Gamma(p, q)$ such that $f\# \gamma' = \bar{\gamma}$. As a result, we have $\Gamma_{\mid \mathbb{B}}(f\#p, f\#q) \subset \{ f\#\gamma \colon \gamma' \in \Gamma(p, q) \}$.
We now finish by noting that any $\bar{\gamma} \in \Gamma_{\mid \mathbb{B}}(f\#p, f\#q)$ can be extended to a $\gamma \in \Gamma(f\#p, f\#q)$ which will have $\gamma(z, z') = 0$ for the extended domain (this follows from the fact that $z \not \in \textrm{Supp}(p)$ implies that $\gamma(z, \cdot) = 0$). As a result, the extended $\gamma$ will have the property,
%
\begin{equation*}
    \int_{(\mathcal{X} \times \mathcal{B}) \times (\mathcal{X} \times \mathcal{B})} c_{\ell}((x, y), (x', y')) \dd \gamma'(f\#p, f\#q)
    =
    \int_{(\mathcal{X} \times \mathcal{Y}) \times (\mathcal{X} \times \mathcal{Y})} c_{\ell}((x, y), (x', y')) \dd \gamma(f\#p, f\#q).
\end{equation*}
Which allows the proof to conclude by taking an infimum over the unrestricted coupling $\Gamma(f\#p, f\#q)$.
}

%\fix{
%The networks generally used in Deep Learning experiments are onto/surjective, whenever the weights are not constrained (during the weight updates). This follows from universal approximation results for Neural Networks \new{[Citation needed.]} We will mention this point in the main text, thank you.
%}
%
%\fix{Alex: UA is something to do with the hypothesis class, not a single hypothesis (or all hypotheses) which is required by Assumption 3. So something more subtle needs to be stated.}
%
%\fix{Alex: Hmm... Maybe surjectivity is technically not needed? I am unsure. I have a weak belief that the assumption actually may not be needed? We can be surjective to a subset of $\mathcal{Y}$. Then, by the proposition, the pushforward will be surjective to transport plans with $\mathcal{Y}$ restricted. This still works as the latter will be a subset of the full transport plan space. I think the correct technical requirement is actually, we require $f$ to have an output $B \subset \mathcal{Y}$ that is a measurable (sub)space; and have $f$ by surjective to that.}


% even if surjectivity would not hold, we can make Lipschitz continuity assumption (e.g. probabilistic lipshitzness of JDOT).

\paragraph{Replies to reviewer 4Jsd.}

We thank the reviewer for the comments and try to answer the raised concerns below.

\fix{The authors need to present more experiments on the proposed bounds, the experiments conducted on larger scale dataset like COCO should be added.}

While the submitted paper proposes only theoretical contributions, we tried to present experimental results that clearly support the conclusions that can be drawn from the theoretical contributions (such as entanglement, effect of label shift, CCA assumption, etc.) \new{[TODO: Discuss the added dataset (tiny Imagenet ?) or argue why it's not necessary]}

\fix{The organization of this paper should be improved, it seems the authors' take all of the proof supporting for the lemmas or theorems in the supplementary materials, thus the relationship of each component can not be clearly revealed. The key proof like Theorem 4.7 should be highlighted in the manuscript for more comfortable reading.}

\fix{Alex: I think the reviewer is potentially asking for two things here. 1. with all the Theorems etc, its hard to see which are key. This can be solved via latex envs (colorbox). 2. is the below response. However, I think this 2nd point also stressed the relationship between the results.}

% space permitting
Due to space considerations, we decided to comment out our proof sketches, which clearly indicate the direction of the proofs. For instance for the proof sketch of Lemma 2 (which is a key Lemma in order to understand the paper), we wrote that:

"To prove the lower bounds, we relate the optimal coupling between the joint distributions to the optimal coupling between the marginals by a transformation that disappears once we lower bound the joint cost $c$ with the marginal cost $c_1$.
% write it better
The proof for the upper bounds hinges on the fact that transports that decompose the optimal coupling between $(x,y) \sim \mu$, $(x', y') \sim \nu$ pairs are sub-optimal: the couplings $\gamma(x,x') \gamma(y, y'| x, x')$ and $\gamma(y,y') \gamma(x, x'| y, y')$ incur a cost that upper bounds the optimal transport cost."

\new{
We agree with the reviews that, space permitting, proof sketches would provide the reader better context of the relation between each result. As such, for at least our key results, we will provide proof sketches and will additionally highlight which intermediary results are being utilized to prove the final result. % For example, Theorem 4.7: The theorem follows from decomposing the prediction entanglement term into ...
}

\fix{Maybe not a full sketch}

%The proof sketches are we think quite useful to understand the introduced framework, without getting bogged down in the details (left in the Appendix). We will include them in the updated manuscript, as we will have one more page allowance. \new{Mention the proof sketch for Theorem 4.7?}

\fix{The caption in Fig. 2 should be more clear, what's the meaning of the images and the red points?}

As we wrote also in our response to reviewer GAmG: in the figure, we tried to show one example association computed by optimal transport in the output space of a convolutional neural network) during the WRR-based adaptation. Optimal Transport associates a female image to a male image, possibly because the network is using spurious features (relying on statistically dominant features such as hair length and shape) to represent these images. 

We agree that the Figure can be improved and will make the necessary modifications.

\fix{It would be better to present more visualization results to verify the effectiveness of the bounds in UDA and entanglement.}

% if he means more plots then point to the appendix - more clearly presented there as an upper bound (for the oracles)
Thank you for the suggestion, do you mean additional plots to illustrate what is happening during the domain matching process? Appendix F includes several additional plots corresponding to the results shown in Tables 1 and 2. If you mean visualization like the one shown in Figure 1, we would like to note that in the Portraits dataset that was used, there are only two classes to predict, which makes visualization easy. For the other datasets, there are more classes, which makes it more difficult to visualize the entanglement that happens during the optimization.

\fix{Some minor related works are missing or described incorrectly}

As we wrote in our reply to other reviewers also, we will enlarge and update the Related Work section to include more recent works (such as those mentioned by the reviewer pBhN.

\paragraph{Reply to reviewer dggm.}

We thank the reviewer for the comments and appreciate the positive evaluation. 

\fix{It would be very interesting to explore if certain assumptions can be relaxed such as 1 \& 2.}

As we wrote also in our response to reviewer GAmG, Section 3.1 does include a sentence on this topic: "Despite this, Assumption 1 can be replaced with an approximate triangle inequality (Crammer et al., 2008) with slight alteration to our results." Section D in the Appendix continues this discussion and details how our results extend to more commonly used loss functions that do not obey triangle inequality. We realize that we did not refer to this section of the Appendix in the main text, we will update the discussion accordingly such that the two discussions are connected. 

As for Assumption 2, without a bounded loss, we would need a guarantee that the loss is effectively bounded for the distributions of interest (source and target). Without an effective bound on the loss, the generalization bounds lose their meaning.

\clearpage

\subsection{TODO (from easiest to hardest)} 
\begin{enumerate}
    \item Include Sugiyama-sensei's comments
    \item Go through the paper again and fix typos
    \item Improve Figure 1, use clearer colors?
    \item Read the reviews fully and summarize requests and clarifications desired
    \item Enable the proof sketches and make sure all lemmas have proof sketches
    \item Add standard deviations and number of runs to Tables 1, 2 and connect to experiments in appendix
    \item Discuss assumptions (metric loss, surjective model) and connect to Approximate Triangle inequality discussion in appendix
    \item Correct proof to Theorem 4.7 (and decide how to present it)    
    \item Extend literature review: compare to three papers mentioned by first reviewer
    (Optional: discuss JDOT bound, $H \Delta H$-divergence bound in \cite{benDavid2010}, \cite{zhao2019learning} and \cite{johansson2019support} papers critically, comparing to other results.)
    \item Add more baseline algorithms (e.g. reverse KL)
    \item Add more complex dataset like COCO (mini Imagenet?) to experiments
 
\end{enumerate}

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. Yes
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. Not Applicable
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. No. We will release our code if our submission is accepted.
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. Yes
   \item Complete proofs of all theoretical results. Yes, we provide proofs in the appendix. We also have Proof sketches which we decided to omit due to space considerations.
   \item Clear explanations of any assumptions. Yes     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). No, but we will release all code and necessary instructions if our paper is accepted.
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). Yes, in the appendix we give a detailed description.
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). Yes, in the appendix we provide these details.
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). No, but all our results were computed using our work laptops.
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. Yes. In the appendix we cite all the datasets that we used.
   \item The license information of the assets, if applicable. Not Applicable
   \item New assets either in the supplemental material or as a URL, if applicable. Not Applicable
   \item Information about consent from data providers/curators. Not Applicable. All data that we used have permissible licenses and were obtained either by Pytorch or by downloading them from the data provider's website.
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. Not Applicable
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. Not Applicable
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. Not Applicable
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. Not Applicable
 \end{enumerate}

 \end{enumerate}

==> sections/commented_out.tex <==
\section{TO BE REMOVED}

\begin{comment}
\begin{theorem}
    Suppose Assumption~\ref{assum:metric} to~\ref{assum:surjective}, $\GS(a, b, \varepsilon, s)$, and $\PLM(M, \eta)$ hold; and there exists a $l \geq 1$ such that $\min_{y \neq y'} \ell(y, y') > l$. Then,
    %
    \begin{equation*}
        \predentangle(f) \leq \frac{\varepsilon a s (s+1)}{2} + W_{1, \ell}(p_{\rm y}, q_{\rm y}) \cdot \frac{(1-\eta) \cdot L + M}{l}.
    \end{equation*}
\end{theorem}

\fix{
The tighter bound. Maybe just remove in the main text.
\begin{equation*}
    \predentangle(f) \leq 
    \left( (1-\eta) \cdot L + M \right)
    \cdot
    \frac{W_{1, \ell}(p_{\rm y}, q_{\rm y})}{l}
    +
    \frac{\varepsilon a s (s+1)}{2}
    \cdot 
    \left( 
    1 + W_{1, \ell}(p_{\rm y}, q_{\rm y}) \cdot \left( 1 - \frac{1}{l} \right)
    \right).
\end{equation*}
}
\end{comment}

\begin{comment}
\fix{
\begin{proof}
    The entanglement term in eq. \eqref{eq:bound_in_x} can be written as \fix{check if we have to use the pushforwards, Lemma 3.2 does not hold otherwise?}

    \fix{Alex: Think its fine with pushforwards + surjectivity. It more or less allows you to switch (upperbound) between transport with / without the pushforward in integrals}
    
    \begin{align*}
        \labelentangle(f) = \int \gamma(x,x') W_{1, \ell}(p(y \mid f(x)), q(y \mid f(x'))) dx dx' \\
        W_{1, \ell}(p(y \mid f(x)), q(y \mid f(x'))) = \int \pi(y,y') \ell(y,y') dy dy'
    \end{align*}
    for optimal couplings $\gamma(x,x')$ and $\pi(y,y')$ associated to the marginal and conditional W1-distances respectively. Using triangle inequality on the best classifier $f^{\star}$ and the symmetry of the loss function, 
    \begin{align*}
        \ell(y, y') \leq \ell(f^{\star}, y) + \ell(f^{\star}, f^{\star'}) + \ell(f^{\star'}, y')
    \end{align*}
    which when applied to the entanglement term at $f^{\star}$ yields
    \begin{align*}
        \labelentangle(f^{\star}) &\leq \lambda + \int \gamma(x, x')\ell(f^{\star}(x), f^{\star}(x')) dx dx' \\
        &= \lambda + W_{1, \ell}(p(f^{\star}), q(f^{\star}))
    \end{align*}
    Using the same arguments from Lemma~\ref{lem:close-marginals-cda}, we can bound the marginal distance $\bar{W}(f^{\star}) \defeq W_{1, l}(p(f^{\star}), q(f^{\star})) < \kappa + \tfrac{L + l}{l}\delta$, which implies the upper bound can be further bounded as
    \begin{align*}
    \risk_{q}(f^{\star}) \leq \risk_{p}(f^{\star}) + \bar{W}(f^{\star}) + \labelentangle(f^{\star}) \leq \lambda + 2\kappa + \tfrac{L + l}{l}\delta
    \end{align*}
    Plugging in the upper bound of $\lambda$ from Lemma~\ref{lem:close-marginals-cda} yields then the upper bound $4 \kappa + 3 \tfrac{L + l}{l}\delta$.
\end{proof}
}
\end{comment}

\fix{Remove this section after re-writing above.}\\
\fix{Re-read below: what is missing? (a) a stronger notion of the classifier consistency, (b) connecting the first part up to classifier consistency to Lemma 4.3.}

We analyze now the bound in Corollary~\ref{cor0} carefully and discuss how we can use it to analyze UDA and the various optimizers suggested in the literature minimizing surrogate risks.

The next assumption is typically made when proving upper bounds and is also known as the \emph{low-$\lambda$ assumption}~\citep{benDavid2010}. We call it the \emph{conservative} domain adaptation (CDA) assumption. Without this assumption, we cannot hope to find a model that has high accuracy in both domains.
\fix{Cite previous paper referring to it as CDA.}

\begin{definition}
    The \emph{Conservative Domain Adaptation assumption} $\CDA(\lambda)$ holds for $\lambda > 0$ and a hypothesis class $\mathcal{H}$ if $\lambda = \min_{f \in \mathcal{H}} \risk_{p}(f) + \risk_{q}(f)$.
\end{definition}

\paragraph{CDA Assumption.} There is a classifier $f^{*} \defeq f(\theta^{*})$ in hypothesis class $\mathcal{H}$ that has \emph{low} expected risk $\lambda$ on both the source and the target distributions.

We strengthen this assumption below and show that it implies the CDA assumption whenever the distance between the label distributions are small.
\fix{CCA is no longer required in the lemma below. In fact how is it useful at all? Replace with a better assumption that is more integrated with the story.}

\begin{definition}
    The \emph{Close Conditionals Assumption} $\CCA(\alpha)$ holds for $\alpha > 0$ and a hypothesis class $\mathcal{H}$ if there exists a classifier $f \in \mathcal{H}$ such that $\risk_{p}(f) + \max_y W_{1, \ell}(f\# p_{\rm x \mid \rm y}(\cdot \mid y), f\# q_{\rm x \mid \rm y}(\cdot \mid y)) < \alpha$.
\end{definition}

\paragraph{CCA Assumption.} There is a classifier $f^* \defeq f(\theta^*)$ in hypothesis class $\mathcal{H}$ such that $\CCA(\alpha)$ holds for some \emph{low} $\alpha$. The CCA assumption, unlike first appearance is a valid assumption for deep networks with large enough capacity. To see this, take a deep enough feedforward network with $M$ layers that satisfies the CDA assumption. Now we can append a \emph{linear} layer at the end (with same input and output dimensions) that not only preserves $\lambda$ but also brings the conditionals closer. We provide a complete proof of this assertion in the appendix.
% prove this or remove if it is not necessary

\begin{lemma}\label{lem:close-marginals-cda}
    Suppose Assumptions~\ref{assum:semi-metric} to~\ref{assum:surjective} hold, then $\CDA(\lambda)$ holds with $\lambda = 2\alpha + \frac{L + 1}{l} \cdot \delta$.
\end{lemma}
\begin{proof}[Proof Sketch]
    The proof is a consequence of the fact that if the source and target label distributions are close together in Wasserstein distance then the corresponding coupling is concentrated on the diagonals: off diagonal terms are small and by using upper and lower bounds of the loss, we can cap their effect on the target risk using equation~\eqref{eq:bound_in_y}.
\end{proof}

The above Lemma~\ref{lem:close-marginals-cda} shows the heavy price we might have to pay (in terms of loss) for small deviations of the label distributions: small deviations $\delta$, measured in terms of Wasserstein distance, can be amplified up to ${L}/{l}$ times. If the model $f$ outputs probability distributions (i.e. values in the simplex $R^{M}$), then we can use the diameter of the simplex as measured by the metric $\ell(f, f')$ as the bound $L$. \fix{For the lower bound $l$ we note that $y, y'$ are in the simplex and hence $\min_{y \neq y'}l(y,y')$ can be seen as a scaling factor in the proof. Alex: I don't get this statement} 

As a corollary, we note that when the label distributions are equal these factors disappear. \fix{Similar to above comment: update given that Lemma has changed}

\begin{corollary}\label{cor42}
    Suppose $p_{\rm y} = q_{\rm y}$ and $\CCA(\alpha)$ holds for $\alpha > 0$. Then $\CDA(\lambda)$ holds for $\lambda = 2 \alpha$.
\end{corollary}

\fix{Add reference and context.}
Next we show that this implies an approximate notion of \emph{classifier-consistency}, borrowed from label-noise research to designate risk functions that have nice properties.

\fix{Alex: Is this typically called a "risk function"? From what I've seen, risk function almost always means a "risk" as per ERM / risk minimization (no regularization). "Objective function" is typically use to describe a general minimization target.}
\begin{definition}
    A risk function $R(f)$ is (target) classifier-consistent if $f_{R}^\star \in \arg\min_f R(f)$ implies that $f_R^\star \in \arg\min_f \risk_{q}(f)$. 
\end{definition}

We relax this definition to an approximate notion below, as it is not possible to prove this property of upper bounds in general. %without access to target labels.
\fix{if you have target labels - can you prove it for surrogate risk + entanglement?}

\fix{Alex: To check, but this does not seem like a notion of classifier-consistency. My reasoning is that an approximate version of CC should say something about optimal models being close \wrt the \emph{same} risk / objective, not differing ones.}
\begin{definition}
    A risk function $R(f)$ is $\eta$-classifier consistent if for any $f_{R} \in \arg\min_f R(f)$ and $f_q \defeq \arg\min_f \risk_q(f)$, the target risk is $\eta$-close $\vert \risk_q(f_q) - R(f_{R}) \vert \leq \eta$.
\end{definition}

\fix{Alex: A word on terminology, usually "surrogate" in this context refers to a loss function dominating another. This is typically separate from regularization (which I would maybe argue the Wasserstein distances are).}

Using this approximate notion we can say something about the surrogate risk $R(f) \defeq \risk_p(f) + W_{1, \ell}(f \# p_x, f \# q_x)$: if we can minimize it, then its minimum value does not exceed the best target risk by more than $\lambda$. We refer to its minimizer as $f_{R}$ below.

\fix{Alex: I don't see why this result requires $\CCA$. Small source risk is likely all you require.}

\fix{Alex: Ok, I don't think this result is useful after carefully looking into this.

1. The proof is broken. The inequalities below do not imply a bound on the different in risks.
Although one \emph{can} get a bound using the exact same proof method as Lemma~\ref{lem:close-marginals-cda}.

2. However, from the listed bound, and the "fixed" bound, we are getting a result for the "best" $f_R^\star$ but achieving a bound that is equivalent to considering the worse possible $f$, \ie, the proof technique of Lemma~\ref{lem:close-marginals-cda}. Thus, the proof statement doesn't say anything. Basically it is saying that the $\eta$-classifier-consistency is achievable with $\eta$ set to a bound of the worse possible classifier.


Sketch on the above, basically, utilizing the proof of Lemma~\ref{lem:close-marginals-cda}, we have
%
\begin{equation*}
    0 \leq \risk_q(f) \leq \alpha + \left( \frac{L + 1}{l} \right) \cdot \delta.
\end{equation*}
Then subtracting a different classifier $f'$, we have
%
\begin{equation*}
    \alpha + \left( \frac{L + 1}{l} \right) \cdot \delta
    \leq 
    \risk_q(f) - \risk_q(f')
    \leq
    \alpha + \left( \frac{L + 1}{l} \right) \cdot \delta.
\end{equation*}
Then we just take the "optimal" classifiers to yield the weak result.


\begin{lemma}\label{lemma42}
Whenever $\CCA(\alpha)$ is satisfied for some small $\alpha$ and the W-distance between the label distributions $W_{1, \ell}(p_y, q_y) \leq \delta$ for some small $\delta > 0$, the surrogate risk $R(f) \defeq \risk_p(f) + W_{1, \ell}(f \# p_x, f \# q_x)$ is $\eta$-classifier consistent for $\eta = 2\alpha + B\delta$ for $B = \frac{L + 1}{l}$.
\end{lemma}
%
\begin{proof}
    Using the first lower and upper bounds in Lemma~\ref{lemma2} for 1-Wasserstein distances for any $f \in \mathcal{H}$ the following holds
    \begin{align*}
     \risk_p(f_R) + W_{1,\ell}(f_R \# p_x, f_R \# q_x) &\leq \risk_p(f) + W_{1,\ell}(f \# p_x, f \# q_x) \\
     &\leq \risk_p(f) + \expect_{(y, y') \sim \gamma_{y}^{\star}} \left[W_{1, \ell}(f \# p_{x \mid y}, f \# q_{x \mid y'})\right] + \delta
    \end{align*}
    for the minimizer $f_R$ of the left hand side. Setting $f$ to be the minimizer of the right hand side we get $\min_f R(f) \leq \alpha + B\delta$. Since $\risk_q(f_q) \leq \risk_q(f) \leq \alpha + B\delta$, we get $|\risk_q(f_q) - R(f_R)| \leq \lambda$ for $\lambda \defeq 2\alpha + B\delta$.
\end{proof}
}

However, $\eta$-classifier-consistency of the surrogate risk is not enough for a practical algorithm as the surrogate risk does not upper bound the target risk: the target risk $\risk_q(f_R)$ could be large, since the entanglement term is not known. We need to make additional assumptions about the model or the data generation process in order to keep the entanglement term small, whenever the surrogate risk is small.
\fix{Are we adding alternative assumptions to the PL assumption below?}

\fix{shadowing on $\lambda$ again.}
\paragraph{Probabilistic Lipschitzness Assumption.} A hypothesis $f \in \mathcal{H}$ is Probabilistic Lipschitz (PL) \citep{ben2014domain, courty2017} w.r.t a coupling $\gamma(x,x')$ if given a metric $d(x,x')$, for all $\beta > 0$, $\mathcal{P}_{x, x' \sim \gamma}(\|f(x) - f(x')\| > \beta d(x, x')) < \zeta(\beta)$ for some nonincreasing function $\zeta(\lambda)$. 

% There are many works in the deep learning literature that derive Lipschitz bounds on neural networks. However the difficulty here is to come up with a suitable $\phi$ that is satisfied for the particular neural-network based hypothesis class.

Based on this assumption PL($\beta$), we can analyze the entanglement term and show that \emph{any} intermediate-layer Wasserstein-distance minimization of features necessarily incurs a trade-off between entanglement and the surrogate risk (by pushing up the value of $\lambda$ in CDA($\lambda$). 

\fix{Add small lemma here to show this, copying over arguments from next lemma.}

\paragraph{Modified Surrogate Risk.} Given a DNN $f(x) \defeq f_z \circ g$, (the network is composed of a feature extractor $g(\theta): x \to z$ and a classifier $f_z(\phi): z \to \hat{y}$) we define the modified surrogate risk (MSR) as $R_{\beta}(f) \defeq \risk_{p}(f) + W_{1, \ell}(f \# p_x, f \# q_x) + \beta W_{1, d}(g \# p_x, g \# q_x)$. We refer to the minimizer of $R_{\beta}$ as $f_{\beta} = \arg\min_f R_{\beta}(f)$.

Using the notion of MSR, we show below that this tradeoff can be \emph{beneficial} if the network has enough capacity to enforce low $\lambda$ even when the intermediate layer representations have \emph{shrunk}.

\fix{Alex: This doesn't seem to be using the pushforward OT / transport plan (after using surjectivity). Switch to be consistent with the rest of the paper?}

\fix{Alex: Proof below seems incomplete and incorrect. }
\begin{lemma}
Assume that a network has sufficient capacity to satisfy for some $\lambda > 0$ the $\CDA(\lambda)$ assumption for the optimal classifier $f^{\star}$ having at each layer Wasserstein distances $\bar{W}_k \defeq W_{1,d}(g^{\star}_{k} \# p_x, g^{\star}_{k} \# q_x)$. Then for all intermediate layers $k = 1, \ldots, K-1$ if $W_{1,d}(g^{R}_k \# p_x, g^{R}_k \# q_x) > \bar{W}_k$ there exists some $\beta(k) > 0$ such that $E(f_{\beta}) < E(f_R)$.
\end{lemma}

% Can we show that other related divergence minimization frameworks also incur the same tradeoff? (by bounding with W-distance?)
% Next we analyze the bound in JDOT and show the tradeoff that is incurred when we make the PL assumption.

% Update notation and write properly
\begin{proof}
    The entanglement term in eq. \eqref{eq:bound_in_x} can be written as 
    \begin{align*}
        E(f) &= \int \gamma(x,x') W_{1, l}(p(y \mid f(x)), q(y \mid f(x'))) dx dx' \\
        W_{1, l}(p(y \mid f(x)), q(y \mid f(x'))) &= \int \pi(y,y') l(y,y') dy dy'
    \end{align*}
    for optimal couplings $\gamma(x,x')$ and $\pi(y,y')$ associated to the marginal and conditional W1-distances respectively. Using triangle inequality on the best classifier $f^{\star}$ and the symmetry of the loss function, 
    \begin{align*}
        \ell(y, y') \leq \ell(f^{\star}, y) + \ell(f^{\star}, f^{\star}') + \ell(f^{\star}', y')
    \end{align*}
    which when applied to the entanglement term yields
    \fix{What is $\lambda(\theta)$?}
    \begin{align*}
        E(f_z \circ g_{\theta}) &\leq \lambda(\theta) + \int \gamma(x, x') \ell(f^{\star}(x), f^{\star}(x')) dx dx' \\
        & \leq \lambda(\theta) + \zeta(\beta) + \beta \int \gamma(x, x') d(g(x), g(x')) dx dx' \\
        & = \lambda(\theta) + \zeta(\beta) + \beta W_{1,d}(g_{\theta} \# p_x, g_{\theta} \# q_x) 
    \end{align*}
    where we applied the PL($\beta$) assumption. \fix{$\lambda(\theta)$ by definition will not increase until $W_{1,d}(\cdot)$ hits $\bar{W}_k$; Alex: I don't understand how this is true. From my calculations, $\lambda(\theta)$ should be over the \emph{entire} model $f$}. The optimized $W_{1,d}$ value at $f_{\beta}$ depends smoothly on the parameter $\beta$, hence there exists a $\beta$ small enough to decrease $E(f_{\beta})$ below $E(f_{0}) = E(f_{R})$.
    
    \fix{Alex: I am not convinced in this proof. 
    
    1. There are missing Lipschitz continuity assumptions / inequalities.
    
    2. We should make it clear what the entanglement term is. I've made a definition block, but it uses pushforwards. I've tried doing this for the current definition and it does not work. So we might need to switch to Wasserstein distances on $(x, y)$ with \emph{composed} cost function $f \circ \ell$.
    
    3. The last line does not imply the conclusion. In particular, the previous series of inequalities provide an upper bound on the entanglement. But the reliance on $\beta$ will not translate into the LHS entanglement term, it will only affect the upper bound.}
\end{proof}
\fix{Above applies for \emph{any} coupling so $\gamma$ can be updated once $d(g(x), g(x'))$ is added to the cost function.}

%\fix{Alex: my attempt with pushforwards. Does not work. So you need to use the "before surjective" style of proof for this. I have this result, but it just ends up being JDOT's inequality.}
%
%\begin{proof}
%    Consider the label entanglement function $\predentangle(f)$. The entanglement term consists of an integration of individual Wasserstein distances $W_{1, \ell}(p_{\rm y \mid f}(\cdot \mid \hat{y}), q_{\rm y \mid f}(\cdot \mid \hat{y}'))$ over all $\hat{y}, \hat{y}' \in \mathcal{Y}$ combinations.
%    Fix $\hat{y}, \hat{y}'$ for now. Letting $\gamma^\star_{\rm y}(\cdot \mid \hat{y}, \hat{y}') \in \Gamma(p_{\rm y \mid f}(\cdot \mid \hat{y}), q_{\rm y \mid f}(\cdot \mid \hat{y}'))$ denote the optimal transport plan witnessing the Wasserstein distance.
%    Then we have,
%    %
%    \begin{align*}
%        &W_{1, \ell}(p_{\rm y \mid f}(\cdot \mid \hat{y}), q_{\rm y \mid f}(\cdot \mid \hat{y}')) \\
%        &= \int \ell({y}, {y}') \dd \gamma^\star_{\rm y}({y}, {y}' \mid \hat{y}, \hat{y}') \\
%        &\leq \int \left( \ell(\hat{y}, {y}) + \ell(\hat{y}, \hat{y}') + \ell(\hat{y}', {y}') \right) \dd \gamma^\star_{\rm y}({y}, {y}' \mid \hat{y}, \hat{y}') \\
%        &= \int \ell(\hat{y}, {y}) \dd p_{\rm y \mid f}(y, \hat{y}) +
%        \int \ell(\hat{y}', {y}') \dd q_{\rm y \mid f}(y', \hat{y}') +
%        \ell(\hat{y}, \hat{y}').
%    \end{align*}
%    Now computing the full entanglement term, we have
%    \begin{align*}
%        \predentangle(f)
%        &\leq \int \gamma^\star_{f}(\hat{y}, \hat{y}') \cdot  \left( \int \ell(\hat{y}, {y}) \dd p_{\rm y \mid f}(y, \hat{y}) +
%        \int \ell(\hat{y}', {y}') \dd q_{\rm y \mid f}(y', \hat{y}') +
%        \ell(\hat{y}, \hat{y}') \right) \dd (\hat{y}, \hat{y}')
%        \\
%        &= \int \ell(\hat{y}, {y}) \dd (f\#p)(\hat{y}, y) +
%        \int \ell(\hat{y}', {y}') \dd (f\#q)(\hat{y}', y') +
%        \int \ell(\hat{y}, \hat{y}') \dd \gamma^\star_{f}(\hat{y}, \hat{y}') \\
%        &= \int \ell(f(x), {y}) \dd p(x, y) +
%        \int \ell(f(x'), {y}') \dd q(x', y') +
%        \int \ell(\hat{y}, \hat{y}') \dd \gamma^\star_{f}(\hat{y}, \hat{y}') \\
%        &= \risk_p(f) + \risk_q(f) +
%        \int \ell(\hat{y}, \hat{y}') \dd \gamma^\star_{f}(\hat{y}, \hat{y}')
%    \end{align*}
%\end{proof}

% Commenting out below for now
\begin{comment}

\fix{
    Alex:
    Related to probabilistic Lipschitzness from JDOT?
}  

\paragraph{Related Conditionals Assumption.} The conditional distributions $p(x|y)$ and $q(x|y)$ are connected, either (a) causally, in the sense that $q(x|y) = T_y \# p(x|y)$ for some transform $T(y)$ or through gradual shift: $q(x|y) = \sum_i \alpha_i q_i(x|y)$ is a mixture distribution that can be ordered via Wasserstein distance w.r.t $p(x|y)$ for each class $y$: $W_1(p(x|y), q_{0}(x|y) \leq \epsilon$ and $W_1(q_i(x|y), q_{i+1}(x|y)) \leq \epsilon$ for some small $\epsilon$. We call this the RCA assumption below.
% Discuss this assumption, mention MNIST-M and USPS.

The following lemma shows that under the above two assumptions, the entanglement term is small whenever the surrogate risk is small.

\begin{lemma}
  Under the CCA and the RCA assumptions, there exists a threshold $\tau$ such that whenever the surrogate risk is less than $\epsilon$ then the entanglement term is $\mathcal{O}(\epsilon)$ for $0 < \epsilon \leq \tau$.
\end{lemma}

\begin{proof}
  Sketch: since the regularized source risk is small, the conditionals $p(x|y)$ are clustered well, up to some $\epsilon_1$. Since the Wasserstein distance between $p(x)$ and $q(x)$ are small, $q(x)$ is also clustered up to $\epsilon_1 + \epsilon_2$. Now assume $q(x|y)$ are not clustered: i.e. there is some $y$ closer to $p(x|y')$ than to $p(x|y)$, $y' \neq y$. However for a network with Lipschitz bound $M$, this violates the CCA assumption.
\end{proof}

We can then guarantee that the target risk of the surrogate risk minima is $\lambda$-close to the target risk minima. This is a stronger notion than the $\lambda$-classifier consistency.

\paragraph{Definition.} A risk function $R(f)$ is $\lambda$-risk consistent if for $f_{R} \defeq \arg\min_f R(f)$, $|\risk_q(f_R) - R(f_{R})| \leq \lambda$.

Finally as the main theorem of the paper we show that the surrogate risk is $\lambda$-classifier-consistent.

\begin{theorem}
  Under the RCA and the CCA assumptions, the surrogate risk $\risk_p(f) + W_{1,l}(f \# p_x), f \# q_x)$ is $\lambda$-risk-consistent.
\end{theorem}

\begin{proof}
Use the above lemma.
\end{proof}

Unfortunately a naive minimization of the surrogate risk can fail, as we show below.

\begin{lemma}
A stochastic gradient descent algorithm able to avoid bad local minima of the source loss minimization can get stuck in the surrogate risk minimization.
\end{lemma}

\begin{proof}
  Sketch: (i) show that the gradient of the source loss and the gradient of the Wasserstein distance can counteract each other whenever source-target conditionals are entangled. \\
  (ii) we can construct a case where SGD able to avoid local minima that have Hessians with maximum eigenvalue bounded by $\lambda_{\max}$ can get stuck as $\lambda_{\max}$ can grow arbitrarily high depending on the degree of entanglement.
\end{proof}

This suggests that depending on the (model, optimizer, data) triplet, one can see very different behaviour of UDA algorithms minimizing source loss together with a divergence term. In practice, depending on the samples, the cost function might plateau or show bounded oscillations around a set value.

\subsection{Algorithm}

Based on the above considerations, we consider an algorithm which guarantees that the marginal divergence is \emph{always} small, hence avoiding the local minima of the usual upper bound minimization algorithms. Given an initial parameter $\theta_0$ which guarantees $W_1(\hat{p}(f_{\theta_0}(x)), \hat{q}(f_{\theta_0}(x)) < \lambda$ for some threshold $\lambda$, we then consider the constrained optimization which minimizes the regularized source loss while respecting the Wasserstein distance between the source and target outputs

\begin{align*}
  \min_{\theta} \emprisk_p(f(\theta)) + \sum_i \gamma_i \mathrm{tr}(\Sigma_i(f(\theta))) \ \mathrm{s. t} \\
  W_1(\hat{p}(f(x)), \hat{q}(f(x))) \leq \lambda
\end{align*}

Initially we may want to set $\lambda$ high and then anneal it over the epochs as we minimize the regularized source risk.

\end{comment}
